Cooperation Does Matter: Exploring Multi-Order Bilateral Relations for Audio-Visual Segmentation

Recently, an audio-visual segmentation (AVS) task has been introduced, aiming to group pixels with sounding objects within a given video. This task necessitates a first-ever audio-driven pixel-level understanding of the scene, posing significant challenges. In this paper, we propose an innovative audio-visual transformer framework, termed COMBO, an acronym for COoperation of Multi-order Bilateral relatiOns. For the first time, our framework explores three types of bilateral entanglements within AVS: pixel entanglement, modality entanglement, and temporal entanglement. Regarding pixel entanglement, we employ a Siam-Encoder Module (SEM) that leverages prior knowledge to generate more precise visual features from the foundational model. For modality entanglement, we design a Bilateral-Fusion Module (BFM), enabling COMBO to align corresponding visual and auditory signals bi-directionally. As for temporal entanglement, we introduce an innovative adaptive inter-frame consistency loss according to the inherent rules of temporal. Comprehensive experiments and ablation studies on AVSBench-object (84.7 mIoU on S4, 59.2 mIou on MS3) and AVSBench-semantic (42.1 mIoU on AVSS) datasets demonstrate that COMBO surpasses previous state-of-the-art methods. Code and more results will be publicly available at https://yannqi.github.io/AVS-COMBO/.

==> bib_copy.tex <==











@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})


@ARTICLE{2022_eombdiedAI,
  author={Duan, Jiafei and Yu, Samson and Tan, Hui Li and Zhu, Hongyuan and Tan, Cheston},
  journal={IEEE Transactions on Emerging Topics in Computational Intelligence}, 
  title={A Survey of Embodied AI: From Simulators to Research Tasks}, 
  year={2022},
  volume={6},
  number={2},
  pages={230-244},
  doi={10.1109/TETCI.2022.3141105}}


@inproceedings{2020vggsound,
  title={Vggsound: A large-scale audio-visual dataset},
  author={Chen, Honglie and Xie, Weidi and Vedaldi, Andrea and Zisserman, Andrew},
  booktitle={ICASSP},
  pages={721--725},
  year={2020},
  organization={IEEE}
}

@article{2016soundnet,
  title={Soundnet: Learning sound representations from unlabeled video},
  author={Aytar, Yusuf and Vondrick, Carl and Torralba, Antonio},
  journal={NIPS},
  volume={29},
  year={2016}
}

@inproceedings{2017looklisten,
  title={Look, listen and learn},
  author={Arandjelovic, Relja and Zisserman, Andrew},
  booktitle={ICCV},
  pages={609--617},
  year={2017}
}

@inproceedings{2018learningSSL,
  title={Learning to localize sound source in visual scenes},
  author={Senocak, Arda and Oh, Tae-Hyun and Kim, Junsik and Yang, Ming-Hsuan and Kweon, In So},
  booktitle={CVPR},
  pages={4358--4366},
  year={2018}
}

@inproceedings{2021localizingSSL,
  title={Localizing visual sounds the hard way},
  author={Chen, Honglie and Xie, Weidi and Afouras, Triantafyllos and Nagrani, Arsha and Vedaldi, Andrea and Zisserman, Andrew},
  booktitle={CVPR},
  pages={16867--16876},
  year={2021}
}


@inproceedings{2022AVS,
  title={Audio--visual segmentation},
  author={Zhou, Jinxing and Wang, Jianyuan and Zhang, Jiayi and Sun, Weixuan and Zhang, Jing and Birchfield, Stan and Guo, Dan and Kong, Lingpeng and Wang, Meng and Zhong, Yiran},
  booktitle={ECCV},
  pages={386--403},
  year={2022},
  organization={Springer}
}


@article{2023AVSS,
  title={Audio-Visual Segmentation with Semantics},
  author={Zhou, Jinxing and Shen, Xuyang and Wang, Jianyuan and Zhang, Jiayi and Sun, Weixuan and Zhang, Jing and Birchfield, Stan and Guo, Dan and Kong, Lingpeng and Wang, Meng and others},
  journal={arXiv preprint arXiv:2301.13190},
  year={2023}
}


@article{2023AV-SAM,
  title={AV-SAM: Segment anything model meets audio-visual localization and segmentation},
  author={Mo, Shentong and Tian, Yapeng},
  journal={arXiv preprint arXiv:2305.01836},
  year={2023}
}


@InProceedings{2023_SAM_ICCV,
    author    = {Kirillov, Alexander and Mintun, Eric and Ravi, Nikhila and Mao, Hanzi and Rolland, Chloe and Gustafson, Laura and Xiao, Tete and Whitehead, Spencer and Berg, Alexander C. and Lo, Wan-Yen and Dollar, Piotr and Girshick, Ross},
    title     = {Segment Anything},
    booktitle = {ICCV},
    month     = {October},
    year      = {2023},
    pages     = {4015-4026}
}



@article{2023_bavs,
  title={BAVS: Bootstrapping Audio-Visual Segmentation by Integrating Foundation Knowledge},
  author={Liu, Chen and Li, Peike and Zhang, Hu and Li, Lincheng and Huang, Zi and Wang, Dadong and Yu, Xin},
  journal={arXiv preprint arXiv:2308.10175},
  year={2023}
}

@InProceedings{2023_icml_unidiffuser,
  title = 	 {One Transformer Fits All Distributions in Multi-Modal Diffusion at Scale},
  author =       {Bao, Fan and Nie, Shen and Xue, Kaiwen and Li, Chongxuan and Pu, Shi and Wang, Yaole and Yue, Gang and Cao, Yue and Su, Hang and Zhu, Jun},
  booktitle = 	 {ICML},
  pages = 	 {1692--1717},
  year = 	 {2023},
  editor = 	 {Krause, Andreas and Brunskill, Emma and Cho, Kyunghyun and Engelhardt, Barbara and Sabato, Sivan and Scarlett, Jonathan},
  volume = 	 {202},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {23--29 Jul},
  publisher =    {PMLR},
  pdf = 	 {https://proceedings.mlr.press/v202/bao23a/bao23a.pdf},
  url = 	 {https://proceedings.mlr.press/v202/bao23a.html},
}


@article{2023_leveraging,
  title={Leveraging Foundation models for Unsupervised Audio-Visual Segmentation},
  author={Bhosale, Swapnil and Yang, Haosen and Kanojia, Diptesh and Zhu, Xiatian},
  journal={arXiv preprint arXiv:2309.06728},
  year={2023}
}

@article{2023gavs,
  title={Prompting Segmentation with Sound is Generalizable Audio-Visual Source Localizer},
  author={Wang, Yaoting and Liu, Weisong and Li, Guangyao and Ding, Jian and Hu, Di and Li, Xi},
  journal={arXiv preprint arXiv:2309.07929},
  year={2023}
}

@article{2023avsegformer,
  title={Avsegformer: Audio-visual segmentation with transformer},
  author={Gao, Shengyi and Chen, Zhe and Chen, Guo and Wang, Wenhai and Lu, Tong},
  journal={arXiv preprint arXiv:2307.01146},
  year={2023}
}

@article{2023catr,
  title={Catr: Combinatorial-dependence audio-queried transformer for audio-visual video segmentation},
  author={Li, Kexin and Yang, Zongxin and Chen, Lei and Yang, Yi and Xun, Jun},
  journal={arXiv preprint arXiv:2309.09709},
  year={2023}
}

@article{2023improving,
  title={Improving audio-visual segmentation with bidirectional generation},
  author={Hao, Dawei and Mao, Yuxin and He, Bowen and Han, Xiaodong and Dai, Yuchao and Zhong, Yiran},
  journal={arXiv preprint arXiv:2308.08288},
  year={2023}
}


@InProceedings{2022_CVPR_GLIP,
    author    = {Li, Liunian Harold and Zhang, Pengchuan and Zhang, Haotian and Yang, Jianwei and Li, Chunyuan and Zhong, Yiwu and Wang, Lijuan and Yuan, Lu and Zhang, Lei and Hwang, Jenq-Neng and Chang, Kai-Wei and Gao, Jianfeng},
    title     = {Grounded Language-Image Pre-Training},
    booktitle = {CVPR},
    month     = {June},
    year      = {2022},
    pages     = {10965-10975}
}


@inproceedings{2023_CVPR_generative,
  title={Generative semantic segmentation},
  author={Chen, Jiaqi and Lu, Jiachen and Zhu, Xiatian and Zhang, Li},
  booktitle={CVPR},
  pages={7111--7120},
  year={2023}
}


@INPROCEEDINGS{2017_vggish,
  author={Hershey, Shawn and Chaudhuri, Sourish and Ellis, Daniel P. W. and Gemmeke, Jort F. and Jansen, Aren and Moore, R. Channing and Plakal, Manoj and Platt, Devin and Saurous, Rif A. and Seybold, Bryan and Slaney, Malcolm and Weiss, Ron J. and Wilson, Kevin},
  booktitle={ICASSP}, 
  title={CNN architectures for large-scale audio classification}, 
  year={2017},
  volume={},
  number={},
  pages={131-135},
  doi={10.1109/ICASSP.2017.7952132}}


@inproceedings{2021_DN_DETR,
title={Deformable {\{}DETR{\}}: Deformable Transformers for End-to-End Object Detection},
author={Xizhou Zhu and Weijie Su and Lewei Lu and Bin Li and Xiaogang Wang and Jifeng Dai},
booktitle={ICLR},
year={2021},
url={https://openreview.net/forum?id=gZ9hCDWe6ke}
}

@INPROCEEDINGS{2022_Mask2Former,
  author={Cheng, Bowen and Misra, Ishan and Schwing, Alexander G. and Kirillov, Alexander and Girdhar, Rohit},
  booktitle={CVPR}, 
  title={Masked-attention Mask Transformer for Universal Image Segmentation}, 
  year={2022},
  volume={},
  number={},
  pages={1280-1289},
  doi={10.1109/CVPR52688.2022.00135}}


@INPROCEEDINGS{2016_dice_loss,
  author={Milletari, Fausto and Navab, Nassir and Ahmadi, Seyed-Ahmad},
  booktitle={Fourth International Conference on 3D Vision (3DV)}, 
  title={V-Net: Fully Convolutional Neural Networks for Volumetric Medical Image Segmentation}, 
  year={2016},
  volume={},
  number={},
  pages={565-571},
  doi={10.1109/3DV.2016.79}}


@article{2023_semanticsam,
  title={Semantic-sam: Segment and recognize anything at any granularity},
  author={Li, Feng and Zhang, Hao and Sun, Peize and Zou, Xueyan and Liu, Shilong and Yang, Jianwei and Li, Chunyuan and Zhang, Lei and Gao, Jianfeng},
  journal={arXiv preprint arXiv:2307.04767},
  year={2023}
}


@article{2023_lisa,
  title={Lisa: Reasoning segmentation via large language model},
  author={Lai, Xin and Tian, Zhuotao and Chen, Yukang and Li, Yanwei and Yuan, Yuhui and Liu, Shu and Jia, Jiaya},
  journal={arXiv preprint arXiv:2308.00692},
  year={2023}
}


@article{2023_mobile_sam,
  title={Faster Segment Anything: Towards Lightweight SAM for Mobile Applications},
  author={Zhang, Chaoning and Han, Dongshen and Qiao, Yu and Kim, Jung Uk and Bae, Sung-Ho and Lee, Seungkyu and Hong, Choong Seon},
  journal={arXiv preprint arXiv:2306.14289},
  year={2023}
}


@INPROCEEDINGS{2023_Audioset,
  author={Gemmeke, Jort F. and Ellis, Daniel P. W. and Freedman, Dylan and Jansen, Aren and Lawrence, Wade and Moore, R. Channing and Plakal, Manoj and Ritter, Marvin},
  booktitle={ICASSP}, 
  title={Audio Set: An ontology and human-labeled dataset for audio events}, 
  year={2017},
  volume={},
  number={},
  pages={776-780},
  doi={10.1109/ICASSP.2017.7952261}}

@INPROCEEDINGS{2016_Resnet,
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={CVPR}, 
  title={Deep Residual Learning for Image Recognition}, 
  year={2016},
  volume={},
  number={},
  pages={770-778},
  doi={10.1109/CVPR.2016.90}
}


@InProceedings{2020_MSSL,
author="Qian, Rui
and Hu, Di
and Dinkel, Heinrich
and Wu, Mengyue
and Xu, Ning
and Lin, Weiyao",
editor="Vedaldi, Andrea
and Bischof, Horst
and Brox, Thomas
and Frahm, Jan-Michael",
title="Multiple Sound Sources Localization from Coarse to Fine",
booktitle="Computer Vision -- ECCV 2020",
year="2020",
publisher="Springer International Publishing",
address="Cham",
pages="292--308",
abstract="How to visually localize multiple sound sources in unconstrained videos is a formidable problem, especially when lack of the pairwise sound-object annotations. To solve this problem, we develop a two-stage audiovisual learning framework that disentangles audio and visual representations of different categories from complex scenes, then performs cross-modal feature alignment in a coarse-to-fine manner. Our model achieves state-of-the-art results on public dataset of localization, as well as considerable performance on multi-source sound localization in complex scenes. We then employ the localization results for sound separation and obtain comparable performance to existing methods. These outcomes demonstrate our model's ability in effectively aligning sounds with specific visual sources. Code is available at https://github.com/shvdiwnkozbw/Multi-Source-Sound-Localization.",
isbn="978-3-030-58565-5"
}




@article{2021_LGVT,
  title={Discriminative sounding objects localization via self-supervised audiovisual matching},
  author={Zhang, Jing and Xie, Jianwen and Barnes, Nick and Li, Ping},
  journal={NIPS},
 volume = {34},
  pages = {15448--15463},
  year = {2021}
}




@article{2022_iGAN,
  title={Generative transformer for accurate and reliable salient object detection},
  author={Mao, Yuxin and Zhang, Jing and Wan, Zhexiong and Dai, Yuchao and Li, Aixuan and Lv, Yunqiu and Tian, Xinyu and Fan, Deng-Ping and Barnes, Nick},
  journal={arXiv preprint arXiv:2104.10127},
  year={2021}
}


@InProceedings{2021_SST,
    author    = {Duke, Brendan and Ahmed, Abdalla and Wolf, Christian and Aarabi, Parham and Taylor, Graham W.},
    title     = {SSTVOS: Sparse Spatiotemporal Transformers for Video Object Segmentation},
    booktitle = {CVPR},
    month     = {June},
    year      = {2021},
    pages     = {5912-5921}
}

@inproceedings{2020_3dc,
  author       = {Sabarinath Mahadevan and
                  Ali Athar and
                  Aljosa Osep and
                  Laura Leal{-}Taix{\'{e}} and
                  Bastian Leibe and
                  Sebastian Hennen},
  title        = {Making a Case for 3D Convolutions for Object Segmentation in Videos},
  booktitle    = {BMVC},
  publisher    = {{BMVA} Press},
  year         = {2020},
  url          = {https://www.bmvc2020-conference.com/assets/papers/0233.pdf},
  timestamp    = {Wed, 07 Dec 2022 23:13:12 +0100},
  biburl       = {https://dblp.org/rec/conf/bmvc/MahadevanAOLLH20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@InProceedings{2023_ICCV_multimodal,
    author    = {Mao, Yuxin and Zhang, Jing and Xiang, Mochu and Zhong, Yiran and Dai, Yuchao},
    title     = {Multimodal Variational Auto-encoder based Audio-Visual Segmentation},
    booktitle = {ICCV},
    month     = {October},
    year      = {2023},
    pages     = {954-965}
}


@article{2020_discriminative,
  title={Discriminative sounding objects localization via self-supervised audiovisual matching},
  author={Hu, Di and Qian, Rui and Jiang, Minyue and Tan, Xiao and Wen, Shilei and Ding, Errui and Lin, Weiyao and Dou, Dejing},
  journal={NIPS},
  volume={33},
  pages={10077--10087},
  year={2020}
}


@misc{2017_rethinking,
      title={Rethinking Atrous Convolution for Semantic Image Segmentation}, 
      author={Liang-Chieh Chen and George Papandreou and Florian Schroff and Hartwig Adam},
      year={2017},
      eprint={1706.05587},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@ARTICLE{2018_deeplab,
  author={Chen, Liang-Chieh and Papandreou, George and Kokkinos, Iasonas and Murphy, Kevin and Yuille, Alan L.},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={DeepLab: Semantic Image Segmentation with Deep Convolutional Nets, Atrous Convolution, and Fully Connected CRFs}, 
  year={2018},
  volume={40},
  number={4},
  pages={834-848},
  doi={10.1109/TPAMI.2017.2699184}}


@INPROCEEDINGS{2017_PSPNet,
  author={Zhao, Hengshuang and Shi, Jianping and Qi, Xiaojuan and Wang, Xiaogang and Jia, Jiaya},
  booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Pyramid Scene Parsing Network}, 
  year={2017},
  volume={},
  number={},
  pages={6230-6239},
  doi={10.1109/CVPR.2017.660}}

@INPROCEEDINGS{2021_SETR,
  author={Zheng, Sixiao and Lu, Jiachen and Zhao, Hengshuang and Zhu, Xiatian and Luo, Zekun and Wang, Yabiao and Fu, Yanwei and Feng, Jianfeng and Xiang, Tao and Torr, Philip H.S. and Zhang, Li},
  booktitle={2021 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Rethinking Semantic Segmentation from a Sequence-to-Sequence Perspective with Transformers}, 
  year={2021},
  volume={},
  number={},
  pages={6877-6886},
  doi={10.1109/CVPR46437.2021.00681}}

@INPROCEEDINGS{2021_Segmenter,
  author={Strudel, Robin and Garcia, Ricardo and Laptev, Ivan and Schmid, Cordelia},
  booktitle={2021 IEEE/CVF International Conference on Computer Vision (ICCV)}, 
  title={Segmenter: Transformer for Semantic Segmentation}, 
  year={2021},
  volume={},
  number={},
  pages={7242-7252},
  doi={10.1109/ICCV48922.2021.00717}}

@article{2021_segformer,
  title={SegFormer: Simple and efficient design for semantic segmentation with transformers},
  author={Xie, Enze and Wang, Wenhai and Yu, Zhiding and Anandkumar, Anima and Alvarez, Jose M and Luo, Ping},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={12077--12090},
  year={2021}
}

@article{2021_AOT,
  title={Associating objects with transformers for video object segmentation},
  author={Yang, Zongxin and Wei, Yunchao and Yang, Yi},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={2491--2502},
  year={2021}
}


@article{2022_pvt,
  title={Pvt v2: Improved baselines with pyramid vision transformer},
  author={Wang, Wenhai and Xie, Enze and Li, Xiang and Fan, Deng-Ping and Song, Kaitao and Liang, Ding and Lu, Tong and Luo, Ping and Shao, Ling},
  journal={Computational Visual Media},
  volume={8},
  number={3},
  pages={415--424},
  year={2022},
  publisher={Springer}
}


@inproceedings{chen2019hybrid,
  title={Hybrid task cascade for instance segmentation},
  author={Chen, Kai and Pang, Jiangmiao and Wang, Jiaqi and Xiong, Yu and Li, Xiaoxiao and Sun, Shuyang and Feng, Wansen and Liu, Ziwei and Shi, Jianping and Ouyang, Wanli and others},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={4974--4983},
  year={2019}
}

@INPROCEEDINGS{2015_FCN,
  author={Long, Jonathan and Shelhamer, Evan and Darrell, Trevor},
  booktitle={2015 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Fully convolutional networks for semantic segmentation}, 
  year={2015},
  volume={},
  number={},
  pages={3431-3440},
  doi={10.1109/CVPR.2015.7298965}}


@inproceedings{2015-Unet,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={Medical Image Computing and Computer-Assisted Intervention--MICCAI 2015: 18th International Conference, Munich, Germany, October 5-9, 2015, Proceedings, Part III 18},
  pages={234--241},
  year={2015},
  organization={Springer}
}

@misc{2023diffusionAVS,
      title={Contrastive Conditional Latent Diffusion for Audio-visual Segmentation}, 
      author={Yuxin Mao and Jing Zhang and Mochu Xiang and Yunqiu Lv and Yiran Zhong and Yuchao Dai},
      year={2023},
      eprint={2307.16579},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@inproceedings{kirillov2019panoptic,
  title={Panoptic feature pyramid networks},
  author={Kirillov, Alexander and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={6399--6408},
  year={2019}
}

@inproceedings{li2022panoptic,
  title={Panoptic segformer: Delving deeper into panoptic segmentation with transformers},
  author={Li, Zhiqi and Wang, Wenhai and Xie, Enze and Yu, Zhiding and Anandkumar, Anima and Alvarez, Jose M and Luo, Ping and Lu, Tong},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1280--1289},
  year={2022}
}

@inproceedings{xiong2019upsnet,
  title={Upsnet: A unified panoptic segmentation network},
  author={Xiong, Yuwen and Liao, Renjie and Zhao, Hengshuang and Hu, Rui and Bai, Min and Yumer, Ersin and Urtasun, Raquel},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8818--8826},
  year={2019}
}

@article{cheng2021per,
  title={Per-pixel classification is not all you need for semantic segmentation},
  author={Cheng, Bowen and Schwing, Alex and Kirillov, Alexander},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={17864--17875},
  year={2021}
}

@inproceedings{cheng2022masked,
  title={Masked-attention mask transformer for universal image segmentation},
  author={Cheng, Bowen and Misra, Ishan and Schwing, Alexander G and Kirillov, Alexander and Girdhar, Rohit},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={1290--1299},
  year={2022}
}

@inproceedings{li2023mask,
  title={Mask dino: Towards a unified transformer-based framework for object detection and segmentation},
  author={Li, Feng and Zhang, Hao and Xu, Huaizhe and Liu, Shilong and Zhang, Lei and Ni, Lionel M and Shum, Heung-Yeung},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3041--3050},
  year={2023}
}

@inproceedings{jain2023oneformer,
  title={Oneformer: One transformer to rule universal image segmentation},
  author={Jain, Jitesh and Li, Jiachen and Chiu, Mang Tik and Hassani, Ali and Orlov, Nikita and Shi, Humphrey},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2989--2998},
  year={2023}
}

@inproceedings{carion2020end,
  title={End-to-end object detection with transformers},
  author={Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  booktitle={European conference on computer vision},
  pages={213--229},
  year={2020},
  organization={Springer}
}



@misc{ling2023hear,
      title={Hear to Segment: Unmixing the Audio to Guide the Semantic Segmentation}, 
      author={Yuhang Ling and Yuxi Li and Zhenye Gan and Jiangning Zhang and Mingmin Chi and Yabiao Wang},
      year={2023},
      eprint={2305.07223},
      archivePrefix={arXiv},
      primaryClass={cs.SD}
}



==> figure_tex/supp2_fig_architecture.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=2.0\columnwidth]{figure/supp_figure2_architecture.pdf}
    % \vspace{-0.2cm}
    \caption{
    Framework comparison between the existing mainstream methods~\cite{2022AVS,2023avsegformer,ling2023hear} and our proposed COMBO.
    (a) The framework of the mainstream approaches, which mainly explores the stage of the fusion.
    (b) Our COMBO framework, which simultaneously explores multi-order relations.
    } 
    \label{fig:supp_figure2_architecture}
    % \vspace{-0.5cm}
\end{figure*}

